Non-Stationary Policy Learning for Multi-Timescale Multi-Agent Reinforcement Learning

In multi-timescale multi-agent reinforcement learning (MARL), agents interact across different timescales. In general, policies for time-dependent behaviors, such as those induced by multiple timescales, are non-stationary. Learning non-stationary policies is challenging and typically requires sophisticated or inefficient algorithms. Motivated by the prevalence of this control problem in real-world complex systems, we introduce a simple framework for learning non-stationary policies for multi-timescale MARL. Our approach uses available information about agent timescales to define a periodic time encoding. In detail, we theoretically demonstrate that the effects of non-stationarity introduced by multiple timescales can be learned by a periodic multi-agent policy. To learn such policies, we propose a policy gradient algorithm that parameterizes the actor and critic with phase-functioned neural networks, which provide an inductive bias for periodicity. The framework's ability to effectively learn multi-timescale policies is validated on a gridworld and building energy management environment.

==> sections/ack.tex <==
This work was authored in part by the National Renewable Energy Laboratory (NREL), operated by Alliance for Sustainable Energy, LLC, for the U.S. Department of Energy (DOE) under Contract No. DE-AC36-08GO28308. This work was supported by the Laboratory Directed Research and Development (LDRD) Program at NREL. The views expressed in the article do not necessarily represent the views of the DOE or the U.S. Government. The U.S. Government retains and the publisher, by accepting the article for publication, acknowledges that the U.S. Government retains a nonexclusive, paid-up, irrevocable, worldwide license to publish or reproduce the published form of this work, or allow others to do so, for U.S. Government purposes. 
(A portion of) The research was performed using computational resources sponsored by the Department of Energy's Office of Energy Efficiency and Renewable Energy and located at the National Renewable Energy Laboratory.

==> sections/algorithm.tex <==
\begin{algorithm}
    \caption{A multi-timescale policy gradient algorithm for learning multi-agent $K$-periodic non-stationary policies}
    \label{alg:pg}
    \begin{algorithmic} %[1]
        \STATE \algcomment{Init PFNN actor and critic weights $\theta$ and $\phi$}
        \STATE Broadcast $K = \texttt{LCM}(k_1,\dots,k_N,C)$ to all agents
        \FOR{each training step}
            \STATE Init empty buffer
            \FOR{episode $e = 1$ {\bfseries to} BatchSize}
                \STATE $t = 0$, $s_{t} = $ initial state
                \WHILE{$s_t \ne$ terminal {\bfseries and} $t < T$}
                    \STATE \algcomment{Calculate the current phase}
                    \STATE Let $\triangle_t := t \texttt{ mod}(K)$
                    \FOR{each agent $i$}
                        \STATE \algcomment{Check if agent $i$ should act}
                        \IF{$t \texttt{ mod}( k_i )$ {\bfseries equals} $0$}
                            \STATE Get observation $(o_t^i, \triangle_t)$
                            \STATE Sample $a^i_t \sim \pi^i(o_t^i ; \triangle_t,
                            \theta)$ 
                        \ELSE
                        \STATE Either $a^i_t := $ \texttt{null} or $a^i_{t-1}$
                        \ENDIF
                    \ENDFOR
                    \STATE Use $\mathbf{a}_t$ to get reward $r_t$   
                \STATE $t = t + dt$
                \ENDWHILE
                \STATE Add episode to buffer
            \ENDFOR
            \STATE Collate episodes in buffer into training batch        
            \FOR{$t = T$ {\bfseries down to} $1$}
                \STATE Let $\triangle_t := t \texttt{ mod}(K)$
                \STATE \algcomment{Use a ``target'' PFNN critic $\hat{Q}^{\pi}$}
                \STATE Calculate TD targets $\hat{y}_t$
                \STATE Critic loss: $L_c = \text{MSE}(Q^{\pi}(\mathbf{a}_t,s_t ; \triangle_t, \phi), \hat{y}_t )$
                \STATE Update critic weights $\phi' = \phi - \alpha \nabla L_c$
                \STATE \algcomment{Compute policy gradient with, e.g., COMA}
                \STATE $L_{PG} = \log \pi(\mathbf{a}_t | \mathbf{o}_t ; \triangle_t, \theta) A^{\mathbf{\pi}}(\mathbf{a}_t,s_t ; \triangle_t, \phi)$
                \STATE Update actor weights $\theta' = \theta + \alpha \nabla L_{PG}$
            \ENDFOR
        \ENDFOR
\end{algorithmic}
\end{algorithm}

